Quantum-parallel vectorized data encodings and computations on trapped-ions and transmons QPUs

Compact quantum data representations are essential to the emerging field of quantum algorithms for data analysis. We introduce two new data encoding schemes, QCrank and QBArt, which have a high degree of quantum parallelism through uniformly controlled rotation gates. QCrank encodes a sequence of real-valued data as rotations of the data qubits, allowing for high storage density. QBArt directly embeds a binary representation of the data in the computational basis, requiring fewer quantum measurements and lending itself to well-understood arithmetic operations on binary data. We present several applications of the proposed encodings for different types of data. We demonstrate quantum algorithms for DNA pattern matching, Hamming weight calculation, complex value conjugation, and retrieving an O(400) bits image, all executed on the Quantinuum QPU. Finally, we use various cloud-accessible QPUs, including IBMQ and IonQ, to perform additional benchmarking experiments.

==> results_06_qbart_experiments.tex <==
% !TEX root = main.tex
\subsubsection*{Performance of QBArt on simulated hardware}
\label{sec:qbart_simu}

The following 6 \qbart\  binary input encoding experiments of gradually increasing complexity demonstrate that accurate results can be achieved on the current NISQ device.

For simulated {\it experiment \#5} storing 320 random bits on  5 address  and 10 data qubits  we  varied the number of shots per sequence and study the recovery fidelity. We evaluated the results, shown in \cref{fig:qbart-succ-shots},  using both metrics RVF and RSF for the same 4 choices of the simulated noise levels used previously (see  \cref{tab:noise-model}).
Here, we also used \texttt{Qiskit} and we assumed {\it all-to-all} connectivity. 
 
\cref{fig:qbart-succ-shots}(a) shows the symbol fidelity as a function of the number of shots.
For most of the noise models, the fidelity approaches $1.0$ when $10^3$ shots are used.
The exception occurs with the IBMQ-proxy noise; this noise model is so severe that the fidelity stays very low even if $32\cdot10^3$ shots are used. 
This shot-based simulation also shows that a perfect recovery of the entire input sequence is possible using a moderated number of shots, as shown in \cref{fig:qbart-succ-shots}(b).

%%%%%%%%%%%%%%%%%%%%    F I G   %%%%%%%%%%%%%%%
% QBArt/paper1$ ./pl_shots_fidelity_qbart5+10.py -X
% tab QBart5+10  at  https://docs.google.com/spreadsheets/d/1UjeeYNRaEdIjFfRAU-WbTLyC-zLw95YSwYY5QrKI08s/edit?usp=sharing
\begin{figure}[h!]
\centerline{\includegraphics[width=1\linewidth]{fig/qbart_5+10_shots_fidelity_f44_tp.pdf}}
\caption{Simulated \qbart\ reconstruction fidelity for \qbart\  \textit{experiment \#5} assuming various noise models. (a) single value fidelity (b) whole sequence fidelity. }
\label{fig:qbart-succ-shots}
\end{figure}

To evaluate performance of \qbart\  for a longer realistic sequence, we  generated a synthetic electrocardiogram (ECG) signal, shown in \cref{fig:qbart-cardio}(a). 
The signal was digitized into a sequence of 64 6-bit integers, shown as solid blue in \cref{fig:qbart-cardio}(b).
The \qbart\ \textit{Experiment \#6}  used 6 address qubits and 6 data qubits and was executed on the Quantinuum realistic simulator, H1-1E.
The dashed line in \cref{fig:qbart-cardio}(b) shows the recovered ECG signal. 
Simulating $2\cdot10^3$ shots resulted in the correct recovery of 63 out of the 64 values.  
Based on these results, we expect similar performance when using the real H1-1.

%%%%%%%%%%%%%%%%%%%%    F I G   %%%%%%%%%%%%%%%
% QBArt/paper1$ ./pl_qbart_ECG_paper.py 
\begin{figure}[htbp]
\centerline{\includegraphics[width=.9\linewidth]{fig/qbart-ECG_f1_tp.pdf}}
\caption{Simulated reconstruction of an ECG signal via \textit{experiment \#6}. We use a 12-qubit \qbart\ encoding executed on the Quantinuum H1-1E simulator using $2\cdot10^3$ shots. (a) synthetic ECG signal. (b) digitized input is shown as a solid line and the reconstructed signal is presented as a dashed line.}
\label{fig:qbart-cardio}
\end{figure}
 
 
%%%%%%%%%%%%%%%%% SHORT CIRC different QPUs %%%%%%%%%%%%%%%%%
\subsubsection*{Performance of QBArt on diverse real QPUs}
\label{sec:qbart-ibmq}
As mentioned earlier, \qbart\ generates optimal circuits if a bipartite connectivity is available.
Unlike trapped ions QPUs, the IBMQ and the Rigetti QPUs have mostly 1:2 (linear) with sporadic 1:3 (T-bridges) connectivity, which is not well suited for our \qbart\ encoder.
Nevertheless, we reduce the circuit size by shortening the sequence size and the magnitude of the values to compare the performance of different QPUs in the regime where all types of QPUs have a chance to deliver acceptable results.

\textit{Experiment \#7} encodes 4 random 4-bit values and requires  only 2 address qubits and 4 data qubits. The total number of qubits was 6 and the CX-cycle depth of 8, before the transpilation. 
We executed this experiment on the real QPUs from  Quantinuum, IonQ, IBMQ, and Rigetti.
As reference, we also run the same experiment on the ideal \texttt{Qiskit} simulator and on the Quantinuum H1-1E emulator.
\cref{tab:ibmq-hw} summarizes  the basic characteristics of the used quantum hardware and the number of input sequences.%
%, which was varied depending on  the credits available to us. 
%\rvb{I prefer not to mention that we've had limited access?} \jan{I did it  mainly to justify a different number of input sequences per HW. A natural approach is to run 98 samples on all QPUs. Can you suggest alternative justification?}


%%%%% TTTTTTTTTTTTTTT %%%%%%%%
% Rigetti & IonQ fidelity: arXiv:2203.03816v4
% Rigetti Aspen M-2: https://qcs.rigetti.com/qpus  
% IonQ Aria: https://ionq.com/posts/july-25-2022-ionq-aria-part-one-practical-performance 
\setlength{\tabcolsep}{4pt}
\begin{table}[h!]
%\begin{center}
\begin{tabular}{l|cccc} 
\toprule
& qubits & CX error & CX cycles $\dagger$ & input seq\\
\midrule
 Qantinuum H1 & 20 & 0.003 & 8 & a few \\
 IonQ Harmony & 11 & 0.040 & 8 & a few \\
 IonQ Aria & 23  & 0.004 & 8 & a few \\
 IBM guadalupe & 16 & 0.012 & 42 & 98 \\
IBM montreal & 27 & 0.020 & 39 & 98 \\
IBM jakarta  & 7 & 0.008 & 42 & 98 \\
 Rigetti Aspen-11 & 40 & 0.12 & ~40 & 30 \\ 
 Rigetti Aspen-M-2 & 80 & 0.11 & ~40 & 30 \\ 
\bottomrule
\end{tabular}\\$\dagger$ after transpilation 
%\end{center}
 \caption{Basic characteristics of  quantum hardware  used for  \qbart\ \textit{experiment \#7}. The listed average CX error is officially reported by the hardware providers at the time of circuit execution.}
 \label{tab:ibmq-hw}
\end{table}

The measured fidelity  of  \textit{experiment \#7}  is shown in
\cref{fig:qbart-exp6} as a function of the number of shots. We are not plotting the Rigetti results because of too low fidelity, most likely related to much larger CX-gate error.
%shows the value and sequence fidelity obtained from \textit{experiment \#7} using \qbart\ executed on several types of real QPUs.
The trapped-ion QPUs significantly outperform the transmon-based QPUs. 
The two decisive factors are different  entangling gate fidelity and  versatility of the  native connectivity.
As expected, only for the IBM {\it jakarta}, which has an exceptionally low CX-gate error, we were able to achieve 100\% sequence fidelity using more than $2\cdot10^3$ shots. 
This total number of shots is 100 times higher than an ideal QPU would need, as observed in \cref{fig:qbart-exp6}.
In this experiment, we also analyzed the impact of adding the {\it Dynamical Decoupling} (DD) transpiler pass for IBMQ  QPU and we observed that the fidelity either improved or degraded, depending on a particular QPU; there was no consistent pattern.

%%%%%%%%%%%%%%%%%%%%    F I G   %%%%%%%%%%%%%%%
% QBArt/paper1 ./pl_qbart_ibmq3HW_6Q.py  -X
% Jan owns master macro

\begin{figure}[htbp]
\centerline{\includegraphics[width=1\linewidth]{fig/qbart_ibmq3HW_q2a4d_noDD_f5.pdf}}
\caption{Reconstruction fidelity for \qbart\ experiment \#7 while encoding 4 4-bit integers on 6 qubits, executed on real QPUs provided by  Quantinuum, IonQ, and IBMQ. (a) reconstructed value fidelity (b) reconstructed sequence fidelity. The last H1-1 measurement is for only one input sequence, so no statistical error is presented. }
\label{fig:qbart-exp6}
\end{figure}



%%%%%%%%%%%%%%%%% QTuum long circ %%%%%%%%%%%%%%%%%
\subsubsection*{Performance of QBArt on Quantinuum H1-1}

Our final set of results aims to present the potential of using \qbart\ to perform certain types of data analysis in real hardware, more specifically, using Quantinuum H1-1.
The aim of the three experiments were: calculate the conjugate of a tabulated complex-valued function, perform pattern matching of 2 DNA sequences, and compute the sequence of Hamming weights on an input sequence in integers.

\paragraph{Conjugation operation}

The input to \textit{experiment \#8}
is a tabulated complex exponent:  
\begin{eqnarray}
    \label{eq:csin}
    C_t&=&a \exp{\left[ (b +j c) t +c\right]},    ~~~ C_t \in \mathbb{C},~~~~\text{for}~~~ t \in [0,...,31]\nonumber\\
     A_t, B_t&= &\Re{C_t}, \Im{C_t}, 
\end{eqnarray}
with $j=\sqrt{-1}$ and real parameters $a,b,c,d$ are conveniently chosen to describe an attenuated oscillator with initial values $\abs{A_0},\abs{B_0}\le 2^4 $.
\cref{fig:qbart-exp8} shows the inputs $A(t)$, $B(t)$, and parametric $\{A(t),B(t)\}$ in blue.
%%%%%%%%%%%%%%%%%%%%    F I G   %%%%%%%%%%%%%%%
% H1-1E QBArt/explore   ./ana_qbart_Cspiral_wave.py   --showPlots a  --expName   uusim_d092f1  -p a c  -X
% H1-1 QBArt/explore   ./ana_qbart_Cspiral_wave.py   --showPlots a  --expName   uuexp_fc224b  -p  c   --venue paper   --basePath /dataVault/dataQCrank_2022paper/ -X

\begin{figure}[htbp]
\centerline{\includegraphics[width=.99\linewidth]{fig/uuexp_fc224b_f55.pdf}}
\caption{Results obtained from \textit{experiment \#8} using \qbart\ on a H1-1 QPU are presented in magenta. The input is shown in blue.  (a),(b), and (c) show real, imaginary, and real vs. imaginary components of the complex series, respectively. The conjugation operation performed on QPU only inverted the sign of the imaginary component. Using $10^3$ shots resulted in algebraically accurate results for inputs with entropy of 320 bits.}
\label{fig:qbart-exp8}
\end{figure}

We assign a signed 5-bit representation to both components $A$ and $B$, and we stack them as a single 10-bit value to serve as input to \qbart, as shown in \Cref{circ:qbart-cric8}. 
Next, we apply a bit inversion on $B$ and we recover the output sequence back. 
Only one cycle is needed to invert  all 32 $B_i$ values stored in the Hilbert space.  This circuit uses 5 address qubits and 10 data qubits.
The net result is the computation of the complex conjugate of the input sequence $C_t\rightarrow C^*_t$ on the QPU.
The output $-B_i$ values are {\it 1's complementary} and need to be decoded as such classically, back to {\it signed} integers.
This method of computing 1's complementary was proposed in the original NEQR paper~\cite{Zhang2013a}.
However, to the best of our knowledge, we present the first practical demonstration of such computation using a real QPU. 
To recover all 32 10-bit values {\it exactly}, the  H1-1 required $10^3$ shots. 

%%%%%%%%%%%%%%%%%%%%    CIRCUIT   %%%%%%%%%%%%%%%
\begin{circuit}[h!]
\hspace{1.8cm} % TODO: better solution?
\Qcircuit @C=1.em @R=0.5em {
%QA,  use \raisebox{-4pt}{_5}  to place index below multi-wire line
 \lstick{\ket{0}^{\otimes 5}} &{/}\qw   &\multigate{2}{\qbart(\vec A,\vec B)}  &{/}\qw &  \qw &  \meter & \rstick{i~address} \\
%QB
  \lstick{\ket{0}^{\otimes 5}} &{/}\qw   &\ghost{\qbart(A,B)}  &{/}\qw & \qw &  \meter & \rstick{A_i } \\
 % addr
 \lstick{\ket{0}^{\otimes 5}} &  {/} \qw &\ghost{\qbart(A,B)}   &{/}\qw  \qw & \gate{X}\qw & \meter & \rstick{-B_i }\\
} 
\caption{\qbart\ circuit for \textit{experiment \#8} computing the complex conjugate of the input sequence $(A_t,B_t) \rightarrow (A_t,-B_t)$. The values of $\vec A$ and $\vec B$ are retrieved as {\it signed int} at the addresses  encoded as {\it unsigned int}.}
\label{circ:qbart-cric8}
\end{circuit}



\paragraph{Pattern matching of DNA sequences}
The genetic code of any organism, in short DNA,  is  described as a sequence of {\it codons} that encode  specific amino acids. A codon consist   of three nucleotides.
Since 4 types of nucleotides exist in the Nature there are 64 different codons. To encode an arbitrary base 64 codon  6 classical bits are required. 

On a quantum computer we will use  for this task  6 qubits.
We assigned 2-qubit base states to the 4 nucleotides   as follows: \\
$A=\ket{00},~ T=\ket{01},~ G=\ket{10},~ C=\ket{11}$.\\
Then, any codon   can be encoded  as the tensor product of 3 2-qubit states, denoted $ \ket{a_5...a_0} $.
%  $[\lambda_2,\lambda_1,\lambda_0]
Since we want to compute on a pair of codons A and B  we need 12 qubits,
 labeled $a_0,...,a_5$ and $b_0,...,b_5$, respectively.
 Following  \cref{eq:enc},  the integer value $d \in [4096]$ is combining 2 codons as follows:
\begin{equation}
%d= a_0 + 2a_1+...+2^5 a_5 + 2^6 b_0+ ... +2^{11} b_5
d= \sum_{i=0}^5 2^ia_i + 64 \sum_{i=0}^5 2^ib_i
\label{eq:enc_codon}
\end{equation}
\qbart\ allows to store a sequence of such values as an entangle state. Next, we add  circuitry to compute the {\it exclusive OR} (XOR)  for each pair of input qubits $(a_0,b_0),(a_1,b_1)$, etc. Finally, a sequence of {\it NOT}  and {\it AND}   gates reduces the result to a single  {\it match or no-match} bit, $m_0$. 
The full classical circuit performing  this computation is discussed in more details in~\refmethods.

The quantum \Cref{circ:dna-match} implements  {\it Experiment \#9} performing matching of 2 DNA sequences of length 16.  
We need  the total of 16 qubits, using  12 qubits for codons and  additional 4 to encode the  position in the sequence.
To save on quantum resources, the qubits holding sequence B are `recycled' in the middle of the circuit by applying the {\it reset} gate, which is available on most of QPUs.


%%%%%%%%%%%%%%%%%%%%    CIRCUIT   %%%%%%%%%%%%%%%
\begin{circuit}[h!]
\hspace{0.8cm} % TODO: better solution?
\Qcircuit @C=.4em @R=0.7em {
%addr,  use \raisebox{-4pt}{_5}  to place index below multi-wire line
 \lstick{\ket{0}^{\otimes 4}} &{/}\qw   &\multigate{12}{\rotatebox{90}{\qbart$(~\vec A, \vec B~)$}}  &\qw & \qw   & \qw &  \qw &  \qw   & \qw &  \qw&  \qw &  \qw &  \qw & \qw   & \qw     & \qw  & \qw  &  \meter & &~~addr\\
%QA0
  \lstick{\ket{0}_{a0}} &\qw   &\ghost{Uu}  &\qw &  \targ    & \qw   & \qw & \qw  & \qw   & \qw   & \gate{X} & \ctrl{1} & \qw   & \qw    & \qw  & \qw  & \gate{X}&  \meter & & p_0  \\
%QA1
  \lstick{\ket{0}_{a1}} &\qw   &\ghost{Uu}  &\qw & \qw &  \targ  & \qw   & \qw  & \qw & \qw  & \gate{X} & \ctrl{5} & \qw   & \qw & \qw   & \qw  & \gate{X}  &  \meter & & p_1  \\
%QA2
  \lstick{\ket{0}_{a2}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw  &  \targ  & \qw& \qw & \qw  & \gate{X} & \qw    & \ctrl{1} & \qw    & \qw & \qw   & \gate{X}&  \meter & & p_2    \\
%QA3
  \lstick{\ket{0}_{a3}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw  & \qw &  \targ  & \qw  & \qw  & \gate{X} & \qw    & \ctrl{4} & \qw &\qw  & \qw   & \gate{X} &  \meter & & p_3   \\
%QA4
  \lstick{\ket{0}_{a4}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw  & \qw & \qw &  \targ  & \qw  &   \gate{X}  & \qw   &\qw   &\ctrl{1} & \qw  & \qw  & \gate{X}&  \meter & & p_4 \\
%QA5
  \lstick{\ket{0}_{a5}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw  & \qw & \qw  & \qw &  \targ  &  \gate{X}  & \qw   &\qw    &\ctrl{3} & \qw  & \qw & \gate{X}&  \meter & & p_5 \\
%
%QB0
  \lstick{\ket{0}_{b0}} &\qw   &\ghost{Uu}  &\qw & \ctrl{-6}&  \qw  &  \qw & \qw  & \qw   & \qw  &  \push{\ket{0}}  & \targ &  \qw  & \qw   &\ctrl{2} &\qw  &\qw \\ 
%QB1
  \lstick{\ket{0}_{b1}} &\qw   &\ghost{Uu}  &\qw &  \qw & \ctrl{-6} & \qw & \qw&  \qw  & \qw &    \push{\ket{0}}    & \qw & \targ &  \qw  &\ctrl{2}   &\qw  &\qw  \\
%QB2
  \lstick{\ket{0}_{b2}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw & \ctrl{-6} & \qw & \qw   & \qw  &    \push{\ket{0}}   &  \qw& \qw & \targ &  \qw     &\ctrl{2} &\qw  \\
%QB3
  \lstick{\ket{0}_{b3}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw  & \qw & \ctrl{-6} & \qw    & \qw &    \push{\ket{0}}   &  \qw& \qw &  \qw& \targ  & \ctrl{1} &\qw  \\
%QB4
  \lstick{\ket{0}_{b4}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw  & \qw  & \qw  & \ctrl{-6} &   \qw  &    \push{\ket{0}}  & \qw&   \qw   & \qw & \qw  &\targ &\qw  &     \meter & &m_0 \\
%QB5
  \lstick{\ket{0}_{b5}} &\qw   &\ghost{Uu}  &\qw & \qw  & \qw  & \qw  & \qw  & \qw  & \ctrl{-6} &   \qw   & \qw&   \qw   & \qw & \qw  & \qw  &\qw  \\
% frames
{\gategroup{1}{5}{13}{10}{1.em}{--}}
{\gategroup{1}{12}{12}{16}{0.8em}{--}} \\
    &   \text{state prep}& & & &&\text{XOR} ~\vec A, \vec B   & & & &&&&\text{ AND $\bar p_0,...,\bar p_5$ }
    }
   
\caption{ Quantum circuit evaluating the match between two 16 elements long  input sequence values A and B,  encoded on qubits $a_0,...,a_5$ and  $b_0,...,b_5$,  respectively. The \qbart\ unitary is  preparing the initial state.    The 6 CX gates  compute XOR between bits of sequences element.  The following 5 nested Toffoli gates set the output qubit $m_0$ to state $\ket{1}$ if both 6-bit inputs match. The intermediate XOR output result  is  also measured on qubits $ p_0,...,p_5$.}
\label{circ:dna-match}
\end{circuit}




 {\it Experiment \#9}   was executed  on the real H1-1 QPU. 
The input {\it sequence A} is a random snippet of length 16 from one of the first reported genetic code  of the COVID-19 genome strain~\cite{Sah2020}. 
{\it Sequence B} is a copy of A except  the 5 codons in positions 5 to 10 have been randomly altered, marked in red letters in \cref{fig:dna-parity}.
At the expense of 600 shots and using the majority voting technique, we achieve an exact result for all 16 amino acids. 
It can be observed in \cref{fig:dna-parity}(a) that the 6 XOR bits  $p_0,...,p_5$  are all 0 when 2 codons match, and some of them are non-zero otherwise, following the ground truth. The $m_0$ bit reporting the match is also  correctly computed, as shown in \cref{fig:dna-parity}(b).


%%%%%%%%%%%%%%%%%%%%    F I G   %%%%%%%%%%%%%%%
% emulator H1-1
% QBArt/explore$  ./ana_qbart_Dna_pair.py     --expName    uuexp_d5a88c     --showPlots  c  --venue paper   --basePath /dataVault/dataQCrank_2022paper/  -X


\begin{figure}[htbp]
\centerline{\includegraphics[width=.99\linewidth]{fig/uuexp_d5a88c_f3.pdf}}
\caption{ DNA sequences matching algorithm executed on Quantinuum H1-1 QPU flagged the differences are on positions 5 to 10. (a) 6-bit XOR between codons. (b) final match-bit.  At the expense of 600 shots the exact result was achieved.}
\label{fig:dna-parity}
\end{figure}


\paragraph{Hamming weight computation}
The {\it Hamming distance} between two codons tells in how many places they are different from one another and hence it is an essential tool for studying evolution of the genetic code. 
{\it Hamming weight} of a binary string is defined as the number of  bits set to 1.
In the {\it Experiment \#9} we already computed binary XOR between two codons,  $p_0,...,p_5$, which if passed to the  Hamming weight algorithm  will produce the desired  Hamming distance.

{\it Experiment \#10} computes  Hamming weight on the 3-bit sequence of length 16. We use \qbart\ with 4 address qubits and 3 data qubits to encode the input.
We add 1 {\it ancilla} qubits and the remaining circuitry computing  Hamming weight. The complete quantum \Cref{circ:hammW31} uses 8 qubits, has CX-depth of 28 cycles on a {\it all-to-all} connected QPU. 
The results from  H1-1 measurement on a pseudo-random input sequence and using  300 shots are shown in \cref{fig:qbart-hammW}. 
In this experiments we also match the ground-truth \textit{exactly}.


\Cref{circ:hammW31}   does only 'half' of the job, since it reduce only 3 inputs  $p_0,p_1,p_2$ to 2 output bits $s_0,s_1$. However given enough resources, we could add 2nd copy of the same circuit acting on inputs $p_3,p_4,p_5$ in parallel, next apply some binary adder circuit on two 2-bit inputs to obtain the full Hamming distance between 2 codons.


%%%%%%%%%%%%%%%%%%%%    CIRCUIT   %%%%%%%%%%%%%%%
\begin{circuit}[htbp]
\hspace{1.6cm} % TODO: better solution?
\Qcircuit @C=.9em @R=0.7em {
%addr,  use \raisebox{-4pt}{_5}  to place index below multi-wire line
 \lstick{\ket{0}^{\otimes 4}} &{/}\qw   &\multigate{3}{\qbart}  &\qw & \qw  & \qw &  \qw  & \qw     &  \meter & &~address\\
%QA0
  \lstick{\ket{0}_{p0}} &\qw   &\ghost{\qbart}  &\qw   & \qw   & \qw  &\ctrl{2} &\ctrl{2} &\qw   \\
%QA1
  \lstick{\ket{0}_{p1}} &\qw   &\ghost{\qbart}   &\ctrl{1} &\ctrl{1} &  \qw  & \qw  & \qw  & \qw \\
%QA2
  \lstick{\ket{0}_{p2}} &\qw   &\ghost{\qbart}  &\ctrl{1} & \targ & \qw   &\ctrl{1} & \targ & \meter &  ~s_0 \\
%QB0
  \lstick{\ket{0}} &\qw    &\qw   & \targ   & \qw  &\qw   & \targ   &\qw & \meter &  ~s_1  \\
% frames
    \protect\gategroup{3}{4}{5}{5}{0.8em}{--}   
    \protect\gategroup{2}{7}{5}{8}{0.8em}{--} \\
%   &\\
   &   \text{state prep~~~} &  &~~~~~p_1+p_2  & &&~~~~~~+p_0& \\
}
   \caption{
   Quantum circuit computing the Hamming weight (HW) for a sequence of 16 3-bit integers.  \qbart\ unitary  encodes the input sequence   on qubits $p_i$. The  1st sub-ciruit computes partial HW for inputs $p_1,p_2$. The 2nd one adds the value of $p_0$ to the partial HW stored binary on qubits $s_0,s_1$. The final HWs are measured on qubits $b_0,b_1$ for all addresses.}
\label{circ:hammW31}
\end{circuit}
\newpage
%%%%%%%%%%%%%%%%%%%%    F I G   %%%%%%%%%%%%%%%
% emulator H1-1
% QBArt/explore$  ./ana_qbart_HammWeight.py --showPlots c  --venue paper --expName uuexp_88c221    --basePath /dataVault/dataQCrank_2022paper/ -X

\begin{figure}[htbp]
\centerline{\includegraphics[width=.99\linewidth]{fig/uuexp_88c221_f3.pdf}}
\caption{Hamming weight for a sequence of 16 pseudo-random 3-bit  integers using \Cref{circ:hammW31} executed on Quantinuum H1-1 at the expense of  300 shots.}
\label{fig:qbart-hammW}
\end{figure}


